On Privacy Notions in Anonymous Communication

Many anonymous communication networks (ACNs) with different privacy goals have been developed. However, there are no accepted formal definitions of privacy and ACNs often define their goals and adversary models ad hoc. However, for the understanding and comparison of different flavors of privacy, a common foundation is needed. In this paper, we introduce an analysis framework for ACNs that captures the notions and assumptions known from different analysis frameworks. Therefore, we formalize privacy goals as notions and identify their building blocks. For any pair of notions we prove whether one is strictly stronger, and, if so, which. Hence, we are able to present a complete hierarchy. Further, we show how to add practical assumptions, e.g. regarding the protocol model or user corruption as options to our notions. This way, we capture the notions and assumptions of, to the best of our knowledge, all existing analytical frameworks for ACNs and are able to revise inconsistencies between them. Thus, our new framework builds a common ground and allows for sharper analysis, since new combinations of assumptions are possible and the relations between the notions are known.

==> sections/notions__copy_.tex <==
\section{Protected Properties}
\label{aspects}

%\todo[inline]{Can we start from real life attack and go to the properties by what an adversary can observe? Do we need more explaining for properties? If so, for which?}

We define properties to specify which information is allowed to be disclosed to the adversary, and which must be protected to achieve a privacy notion, as mentioned in Section \ref{background}.
%Intuitively, properties capture information that deliberately is not protected by the \ac{ACN}, like the recipient in Tor~\cite{dingledine04tor}. 
%As explained in Section \ref{background}, we need to define which information is allowed to be disclosed, and which needs to be protected  for the privacy notion by defining properties. Intuitively, properties capture information that can leak while communicating, like e.g. who an active sender is.% capturing the relevant information.
%Hence intuitively, the attack scenarios an adversary can use to break a protocol must be identical regarding these properties.
%If an adversary can construct an attack that can distinguish the two scenarios fulfilling these restrictions, the protocol is broken w.r.t. the notion.
%To formalize these restrictions in our model, we define properties capturing the relevant information.
% Notions can be defined implicitly or explicitly.
%In the implicit case everything in the two scenarios is allowed to change except the defined partial information the adversary is allowed to know.
%In the explicit case everything in the two scenarios has to stay the same except the defined partial information the adversary is not allowed to know. 
  \begin{table}
\center
\resizebox{0.48\textwidth}{!}{%
  \begin{tabular}{ c p{3.5cm} p{4.8cm} }

Symbol &Description&Translation to Game\\ \hline
$|M|$&Message Length& Messages in the two scenarios always have the same length.\\
%$E$&everything &Both scenarios are equal.\\
$\EveryButSender$&Everything but Senders& Everything except the senders is identical in both scenarios.\\
$\EveryButRec/ \EveryButMsg$&Everything but Receivers/Messages& Analogous\\
$\EveryButSenderMsg$&Everything but Senders and Messages& Everything except the senders and messages is identical in both scenarios.\\
$\EveryButReceiverMsg/ \EveryButSenderRec$&Analogous& Analogous\\
 %$\EqualOrNothing$&everything (or nothing is sent)&If something is sent in both scenarios, the communication is the same.\\
\something &Something is sent& In every communication something must be sent ($\Diamond$ not allowed).\\
\nothing &Nothing&Nothing will be checked; always true.\\
$U/U'$& Active Senders/Receivers& Who sends/receives is equal for both scenarios.\\
$Q/Q'$& Sender/Receiver Frequencies&Which sender/receiver sends/receives how often  is equal for both scenarios.\\
$|U|/|U'|$& Number of Senders/ Receivers& How many senders/receivers communicate is equal for both scenarios.\\
$P/P'$& Message Partitioning per Sender/Receiver& Which messages are sent/received from the same sender/receiver  is equal for both scenarios.\\
$H/H'$& Sender/Receiver Frequency Histograms&How many senders/receivers send/receive how often is equal for both scenarios.\\
%$\centernot \rightarrow /\centernot \rightarrow'$& Sender/Receiver absence& some sender/receiver is not participating in any communication in the second scenario.\\
\end{tabular}}
 \caption{Simple properties: Information about communications that may be required to remain private}
  \label{tab:information}
\end{table}

 
 \vspace{-0.3cm}
  \subsection{Simple Properties} 
  \vspace{-0.3cm}
  
  \todo[inline]{"We distinguish between simple and complex properties, where simple properties describe information that intuitively can be observed when communicating and that are easily modeled with the game." -- what does it mean that information can intuitively be observed when communicating?the caption of Figure 1 is a bit vague as well. Your adversary observes whatever the protocol outputs, right? So what does it mean that this information "can be observed but may be required to remain private"? 
  CKu: Tried to change this, but not sure if I made it better or worse...}
  
We distinguish between simple and complex properties, where simple properties describe an intuitive selection of observable information of communications that is easily modeled with the game. We summarize their informal meaning in Table \ref{tab:information}.  

Assume an \ac{ACN}  aims to hide the sender but discloses message lengths to observers. For this case, we specify the property ($|M|$) that the message length must not differ in both scenarios, as this information must not help the adversary to distinguish which scenario the challenger chose to play.

Next, we might want an \ac{ACN} to protect the identity of a sender, as well as any information about who sent a message, but deliberately disclose which messages are received by which receiver,  %have been sent by identical senders, -- this is hidden if senders can differ 
who the receivers are, and potentially other auxiliary information. 
	We hence specify a property ($\EveryButSender$) where only the senders differ in both scenarios\footnote{$E$ symbolizes that only this property may vary in the two submitted scenarios and everything else remains equal.}, to ensure that the adversary in our game can only win by identifying senders. %who the sender of a message actually has been. -- not true, you can also win if you learn the sets of active sender as explained in section 2
The same, of course, has to be defined  for protection of the receivers ($\EveryButRec$) and  of the messages ($\EveryButMsg$).
%Next, we might not want the adversary to learn information about the sender or the sender-message relation. However, it is allowed to link messages, receiver and auxiliary information of the communication. Hence, we need a property to ensure, that only senders can differ in both scenarios. Further, we can require and hence define analogous restrictions for receivers and messages.

Further, we might want the \ac{ACN} to protect senders and in addition also the messages, leaving the receiver and auxiliary information to be disclosed to the adversary. 
This is achieved by specifying a property where only senders and messages differ in the two scenarios and everything else remains equal ($\EveryButSenderMsg$). 
Again, the same is specified for receivers and messages ($\EveryButReceiverMsg$) or senders and receivers ($\EveryButSenderRec$).

Lastly, \ac{ACN}s might allow the adversary to learn whether a real message is sent or even how many messages are sent. Therefore, we specify a property (\something) that requires real communications in both scenarios, i.e. it never happens that nothing is sent in one scenario but something is sent in the other. We ensure this by not allowing the empty communication ($\diamond$).

 However, a very ambitious privacy goal might even require that the adversary learns no information about the communication at all (\nothing). In this case, we allow any two scenarios and check nothing.
 
 \inlineheading{Formalizing those Simple Properties} 
 In the following definition all simple properties mentioned so far are formally defined. 
 %We use $m$ short for certain message, $u$ for a certain sender, $u'$ for certain receiver. For the names of the properties we use $S$ if the senders are treated special, $R$ for receivers, $M$ for the messages and $E_{XY}$ to denote which property may vary, where all others have to remain equal ({\em E(verything except) $XY$}). 
 Therefore, we use $\top$ as symbol for the statement that is always true.
 %An underline denotes a sequence of items, e.g. $\underline{S}$ a sequence of senders. %\todo[inline]{Do I really need to explain this here? Is there a better way?}
 \begin{definition}[Properties $|M|$, $\EveryButSender$, $\EveryButSenderMsg$, \something, \nothing]\label{def:properties} 
 Let the checked batches be $\underline{r_0},\underline{r_1}$,  that include the communications \mbox{${r_0}_j \in \{ (u_{0_j},u'_{0_j},m_{0_j},aux_{0_j}), \diamond\}$} and \mbox{ ${r_1}_j \in \{ (u_{1_j},u'_{1_j},m_{1_j},aux_{1_j}), \diamond\}$} with $ j \in \{1, \dots l\} $. We say the following properties are met, iff for all $j \in \{1, \dots l\}$:
\begin{align*}
   |M|& : |{m_0}_j|=|{m_1}_j| \\[0.5em] %E&: \underline{r}_0 =\underline{r}_1
  \EveryButSender&: {r_1}_j =(\mathbf{u_{1_j}},u'_{0_j},m_{0_j},aux_{0_j}) \\
   \EveryButRec&: {r_1}_j =(u_{0_j},\mathbf{u'_{1_j}},m_{0_j},aux_{0_j}) \\
    \EveryButMsg &: {r_1}_j =(u_{0_j},u'_{0_j},\mathbf{m_{1_j}},aux_{0_j}) \\[0.5 em]
     \EveryButSenderMsg&: {r_1}_j =(\mathbf{u_{1_j}},u'_{0_j},\mathbf{m_{1_j}},aux_{0_j}) \\
   \EveryButReceiverMsg&: {r_1}_j =(u_{0_j},\mathbf{u'_{1_j}},\mathbf{m_{1_j}},aux_{0_j}) \\
   \EveryButSenderRec &: {r_1}_j =(\mathbf{u_{1_j}},\mathbf{u'_{1_j}},m_{0_j},aux_{0_j}) \\[0.5 em]
   % \EqualOrNothing&: {r_0}_j ={r_1}_j \lor {r_0}_j =\Diamond \lor {r_1}_j = \Diamond \\[1em]
 %   E_{a}&: \underline{r_0^a}_j =\underline{r_0^{a'}}_j  \land  \underline{r_1^a}_j =\underline{r_1^{a'}}_j &\forall a, a'& \\
   \text{\something} &: \Diamond \not \in \underline{r}_0 \land \Diamond \not \in \underline{r}_1\\
  \text{\nothing}&: \top
\end{align*}
\label{SimpleProp1}
 \end{definition} 
 
\inlineheading{More Simple Properties: Active Users, Frequencies}
The properties of Definition \ref{SimpleProp1} are important to formalize privacy, but are by itself not sufficient.
Take the \ac{ACN} Tor as an example: While the set of active senders is trivially known to their ISPs and the guard nodes, we still require that the senders are unlinkable with the messages they are sending (and their receivers).
Also the message count a party is sending or receiving is an important information that we cannot formalize so far.
To formalize these properties, we use sets that capture which user sent which messages in a certain period, i.e. a batch of communications (and similarly sets to capture which user received which messages). Note that we use primes for the corresponding sets and properties of the receivers.

\begin{definition}[Sender-Message Linking]\label{def:senderMessageSet}
 We define the sender-message linkings for scenario $b$ ($L'_{b_i}$ the receiver-message linkings analogous) as:
 \begin{align*}
  L_{b_i}:= &\{(u,\{m_1,...,m_h\}) \bigm| u \text { sent messages }m_1, \dots , m_h\\
  &\text{ in batch }i\}\text{.}\\
  \end{align*} 
\end{definition}


The sets from Definition \ref{def:senderMessageSet} easily allow to identify who an active sender in this batch was and how often each of those sent something:

\begin{definition}[Active Sender Set, Frequency Set]\label{UbQb}
Let the current batch be the $k$-th one. % and  $s_{b_i}, s'_{b_i}$ defined as in Definition \ref{def:senderMessageSet}.
For $ b \in \{0,1\}$ $U_b,Q_b$  ($U_b',Q_b'$ for $L_b'$) are defined as:
\begin{align*}
 	U_b &:= \{ u \bigm|  (u,M) \in L_{b_k}\}\hfill\\
        Q_b &:= \{ (u,n) \bigm|  (u,M) \in L_{b_k}\land |M|=n\}\\
\end{align*}
\end{definition}


Recall that we currently define properties for ACNs that allow the adversary to learn which senders are active at different times, or the number of messages they send during some periods while they hide some other properties (e.g. which messages they have sent). 
Hence with the respective sets for active users and user frequencies defined, we only need to request that they are equal in both scenarios:

\begin{definition}[Properties $U$, $Q$, $|U|$]
%Let $U_b , Q_b$ be defined according to Definition \ref{UbQb}.
We say that the properties $U,Q,|U|$ ($U',Q', |U'|$ analogous) are met, iff:
\[U: U_0=U_1 \hspace{1,5em}  Q: Q_0=Q_1  \hspace{1,5em}  |U|: |U_0|=|U_1| \]
\end{definition}  

\inlineheading{More Simple Properties: Message Partitions, Histograms}
Other interesting properties are which messages stem from the same sender or how many senders sent how many messages. If the adversary knows which messages are sent from the same sender, e.g. because of a pseudonym, she might be able to combine information from all of them and identify the sender. If she knows how many senders sent how many messages, she knows the sender activity and hence can make conclusions about the nature of the senders. 

As before, we introduce auxiliary variables to formally define these two properties.
We use $M_{b,I}$ to denote the collection of messages that has been sent by the same sender (e.g. linked by a shared pseudonym) in a set of batches, and $M_{b,I,n}$ to denote the union of all these sets of the cardinality $n$.
The equality of the properties in the two scenarios has to pertain throughout all comparable batches in the scenarios. Otherwise the inequality would help the adversary to distinguish the scenarios without learning the protected information e.g. identifying the sender.
%(if the privacy notion is achieved) and hence must not help her to win the indistinguishability game.%\footnote{Therefore, we use $\mathcal{P}(Z)$ to denote the power set of $Z$.}
%\todo[inline]{you say that the equality would not help the adversary to identify the sender if the notion is achieved. My intuition was the opposite, namely that you define restrictions, because inequality would help the adversary and so you enforce equality in the notion. Maybe its just the wording, but I found this confusing.}

\begin{definition}[Multi-Batch Message Linkings]\label{def:messageSets} Let the current batch be the $k$-th, \mbox{$\mathcal{K}:=\{1, \dots, k\}$}, $\mathcal{P}(\mathcal{K})$ the power set of $\mathcal{K}$ and $\mathcal{U}$ the set of all possible senders ($\mathcal{U'}$ receivers).
 For $b \in \{0,1\}$ and $I \in \mathcal{P}(\mathcal{K})$: We define ($M'_{b,I}, M'_{b,I,n}$ for $L'_{b_i}$)
 \begin{itemize}
 \item the multi-batch-message-sender-linking:\\ \mbox{$M_{b,I} := \cup_{u\in \mathcal{U}} \{ \cup_{i \in I}\{M| (u,M)\in L_{b_i}\}\}$} and
 \item the cardinality restricted multi-batch-message-sender-linking:  $M_{b,I,n}:=\{ M \in M_{b,I} \bigm| |M|=n \}$.
 \end{itemize}
\end{definition}

As before we define auxiliary variables capturing the information that we want to be equal in both scenarios: We define ordered sets specifying which messages are sent from the same user for any set of batches (Message Partition $P_b$) and how many users sent how many messages for any set of batches (Histogram $H_b$).  Therefore, we use a slightly unusual notation: For any set Z, we use $(Z_i)_{i\in\{1,\dots, k\}}$ to denote the sequence $(Z_1, Z_2, \dots, Z_k)$ and $\overrightarrow{\mathcal{P}}(Z)$ to denote a sorted sequence of the elements of the power set\footnote{For brevity we use $\in$ to iterate through a sequence.} of $Z$.
% and `$\_$’ to declare that this part of a tuple can be any value.\footnote{E.g.
%$\exists(S,m,\_) \in r$ will be true iff $\exists R: \exists(S,m,R) \in r$.}
%\todo[inline]{Do we still need $\_$ anywhere?}

%As the challenger checks the properties for every batch of communications, we further need to specify the current batch to be $k$ and $\mathcal{K}$ to include all batches that already have been given to the challenger. 

\begin{definition}[Message partitions, Histograms]\label{def:properties}
 
Consider the $k$-th batch, \mbox{$\mathcal{K}:=\{1, \dots, k\}$}. %and let $M_{b,I},M_{b,I,n}$ be defined as in Definition \ref{def:messageSets} \cts{once you defined it, you don't need to emphasize this anymore...}.
For $ b \in \{0,1\}$  $P_b, H_b$  ($P_b',H_b'$ analogous) are defined as:
 \allowdisplaybreaks
\begin{align*}
	P_b &:= (M_{b,I})_{ I \in \overrightarrow{\mathcal{P}}(\mathcal{K})}\\
	H_b &:= (\{(n, i) \bigm|   i= |M_{b,I,n}|\})_{ I \in \overrightarrow{\mathcal{P}}(\mathcal{K})}\\
\end{align*}

\vspace{-0.5cm}
Further, we say that properties $P,H$ ($P',H' $ analogous) are met, iff:
\begin{align*}
  P&: P_0=P_1 \hspace{3em}  H: H_0=H_1\\
\end{align*}
 \end{definition} 
 %Do we need $\underline{r}_0^a =\underline{r}_0^{a'}$ f.a. $a,a'$? not for simple properties. Even if adv can determine a , its no advntage guessing b, for complex properties we realize this further down

\subsection{Complex Properties}
\label{sec:ComplexProperties}
 \vspace{-0.3cm}
 
So far we defined various properties to protect senders, messages, receivers, their activity, frequency and grouping of messages. 
%So far our scenarios differ in the incidence and frequency of the above properties. \todo[inline]{not sure that the ``incidence and frequency'' really is what simple properties define... but I don't have a better suggestion}
However, this does not suffice to formalize several relevant privacy goals, and we hence introduce complex properties.
 
 %The properties defined so far are sufficient to express many privacy goals. 
% We defined many properties so far. However, there are some typical goals for which we need other properties that are based on additional concepts. Since we need those additional concepts to define them, we call them complex properties.
 
 \inlineheading{Learning Sender and Receiver}
%Complex properties need to add new concepts to the game. We motivate them with an exemplary privacy goal that needs the new concept.
Consider that one aims to hide which sender is communicating with which receiver.
%A typical goal of \acp{ACN} is to hide the relationship between the sender and receiver, i.e. who sends to whom. 
This goal is already used in early \acp{ACN} like the classical Mix-Nets~\cite{chaum81untraceable} and  also in Tor~\cite{dingledine04tor}. Therefore, we want the adversary to win the game only if she identifies both: sender and receiver of the same communication. 

An intuitive solution may be to model this goal by allowing the adversary to pick different senders and receivers ($\EveryButSenderRec$) in both scenarios (see Fig. \ref{fig:senderReceiver} (a) for an example). 
This, however, does not actually model the privacy goal: by identifying only the sender or only the receiver of the communication, the game adversary could tell which scenario was chosen by the challenger. % as the sets of senders and receivers are mutually exclusive, in this case.
%However, this does not work. In fact, any two communications that differ in senders or receivers or both can be distinguished by learning only the sender or only the receiver.  So, we cannot express that sender and receiver have to be learned, without extending the game we defined so far.
We hence have to extend the simple properties and introduce scenario \emph{instances} to model dependencies.

\inlineheadingTwo{Scenario instances}
 We now require the adversary to give alternative instances for both scenarios (Fig. \ref{fig:senderReceiver} (b)). The challenger chooses the scenario of the challenge bit, which is picked randomly for every game, and the instance according to the instance bit, which is picked randomly for every challenge.
 
 Formally, we replace step 2- 5 of the game with the following steps:
 \begin{description}
\item[2.] $\mathcal{A}$ sends a batch query, containing $\underline{r}^0_{0}$,  $\underline{r}^1_{0}$, $\underline{r}^0_{1}$and $\underline{r}^1_{1}$ to $Ch$. 
\item[3.] $Ch$ checks if the query is valid according to the analyzed notion $X$. 
\item[4.] If the query is valid  and $Ch$ has not already picked an instance bit $a$ for this challenge, $Ch$ picks $a \in \{0,1\}$ randomly  and independent of $b$. Then it inputs the batch corresponding to $b$ and $a$ to $\Pi$. 
\item[5.] $\Pi$'s output $\Pi(\underline{r}^a_{b})$ is forwarded to $\mathcal{A}$. 
 \end{description}
% \footnote{Note, that $a \in \{0,1\}$ could easily be replaced by $a \in \{0, \dots, a_{max}\}$ for bigger $a_{max}$, if needed to express other properties.}
 
This allows us to model the goal that the adversary is not allowed to learn the sender and receiver: We allow the adversary to pick two sender-receiver pairs, which she uses as instances for the first scenario. 
The mixed sender-receiver pairs then have to be provided as instances for the second scenario (see Fig. \ref{fig:senderReceiver} (b)). 
We thus force the game adversary to provide alternative assignments for each scenario.
This way she cannot abuse the model to win the game by identifying only the sender or the receiver.
%, despite beinidentifying sender-receiver pairs in the actual protocol, as she cannot distinguish the scenarios by identifying only the sender or only the receiver in this case anymore. 
%One instance of the scenario corresponding to the challenge bit $b$ will be randomly picked. 
We call this property \textit{Random Sender Receiver} $R_{SR}$. 

This complex property still is not sufficient to model the situation in, for example, Tor:
%However,  this is not the correct property: 
The adversary can distinguish the scenarios without learning who sent to whom, just by learning which senders and which receivers are active. 
We hence further restrict the adversary to pick instances where both senders and both receivers are active by defining property \textit{Mix Sender Receiver} $M_{SR}$. 
Here, the adversary picks two instances for $b=0$ where her chosen sender-receiver pairs communicate and two for $b=1$ where the mixed sender-receiver pairs communicate. 
The two instances simply swap the order in which the pairs communicate (Fig. \ref{fig:senderReceiver} (c)). 
This way, we force the adversary to provide alternative assignments  for each scenario where both suspected senders and both suspected receivers are active. 
This combination prevents the adversary to win the game without learning the information that the real system is actually supposed to protect, i.e. the sender-receiver pair. We call this property \textit{Mixed Sender Receiver} $M_{SR}$.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.48\textwidth]{images/complexProp.pdf}
  \caption{Examples showing the general structure of communications that differ in both scenarios: a) Naive, but incorrect b) Random Sender Receiver $R_{SR}$ c) Mixed Sender Receiver $M_{SR}$}
  \label{fig:senderReceiver}
\end{figure}
\inlineheading{Defining Complex Properties}
For an easier formal definition of the complex properties, we introduce \emph{challenge rows}. A challenge row is a pair of communications with the same index that differ in the two scenarios (e.g. ${r}_{0_j}, {r}_{1_j}$ with index $j$). 
For complex properties the challenger only checks the differences of the challenge rows in the two scenarios.
% and hence, only need to consider the challenge rows.

\begin{definition}[Properties $R_{SR}$, $M_{SR}$]\label{def:complexProperties}
Let the given batches be $\underline{r}_b^a$ for instances $a \in \{0,1\}$ and scenarios $b \in \{0,1\}$, 
  $\mathsf{CR}$  the set of challenge row indexes, 
  $(u^a_0, {u'}^{\:a}_0)$ for both instances $a\in \{0,1\}$  be the sender-receiver-pairs of the first challenge row of the first scenario ($b=0$) \iflong in this challenge \fi.
Random Sender Receiver $R_{SR}$, Mixed Sender Receiver $M_{SR}$ ($R_{SM}, R_{RM}, M_{SM}, M_{RM}$ analogous) are met, iff:
\allowdisplaybreaks
\begin{align*}
   R_{SR}:\quad{r_{0}^a}_{cr}&=(\mathbf{u^{a}_0}, \mathbf{{u'}^{\:a}_0}, m^1_{0_{cr}}, aux^1_{0_{cr}})~\land \\
   {r_{1}^a}_{cr}&=(\mathbf{u^{a}_0}, \mathbf{ {u'}^{\:1-a}_0}, m^1_{0_{cr}},aux^1_{0_{cr}})\\[0.2em]
   &\forall cr \in \mathsf{CR} , a \in \{0,1\}&
\end{align*}
\begin{align*}
      M_{SR}:\quad&{r_0^a}_{cr}=(\mathbf{u^{a}_0}, \mathbf{ {u'}^{\:a}_0},m^1_{0_{cr}},aux^1_{0_{cr}})~\land \\
   &{r_0^a}_{cr+1}= (\mathbf{u^{1-a}_0}, \mathbf{ {u'}^{\:1-a}_0}, m^1_{0_{cr}},aux^1_{0_{cr}})~\land \\[0.2em]
   &{r_1^a}_{cr}=(\mathbf{u^{a}_0}, \mathbf{ {u'}^{\:1-a}_0},m^1_{0_{cr}},aux^1_{0_{cr}})~\land \\
   &{r_1^a}_{cr+1}=(\mathbf{u^{1-a}_0},\mathbf{ {u'}^{\:a}_0}, m^1_{0_{cr}},aux^1_{0_{cr}})\\[0.2em]
   &\text{for every second } cr \in \mathsf{CR} , a \in \{0,1\}& 
\end{align*}
%\todo[inline]{The last cr has to skip every second cr.. How to write this?}

\end{definition}
%We do need message and aux fixed even if $a$ changes, otherwise adv could use this to figure out a and knowing a helps to distinguish the scenarios with less information here (e.g. which sender comes first, would then break M_{SR}
 
\inlineheading{Linking message senders}
A last common privacy goal that still cannot be covered is the unlinkability of senders over a pair of messages (\anoaULLong).
Assume a real world adversary that can determine that the sender of two messages has been the same entity.
If subsequently she discovers the identity of the sender of one of the messages through a side channel, she can also link the second message to the same individual.
%Another goal, that we did not cover before, is  that the adversary does not learn whether two messages have the same sender (\anoaULLong). %, see Section \ref{sec:OverviewNotion}). 
%\todo[inline]{I can't think of a example that states this goal...}

\inlineheadingTwo{Stages}
To model this goal, we need two scenarios  (1) both messages are sent by the same sender, and (2) every message is sent by different senders. 
Further, the adversary shall pick the messages, for which she wants to decide whether they are sent from the same individual, and which other messages are sent between those two messages. 
Therefore, we add the concept of \emph{stages} and ensure that only one sender sends in the challenge rows of stage 1 and in stage 2 either the same sender continues sending ($b=0$) or another sender sends those messages ($b=1$). This behavior is specified as the property \emph{Twice Sender} $T_S$. 

%``switch to stage 2'' as message in both scenarios. This communication will be discarded by the challenger and not input to the protocol model. 

%Some notions use stages and require different sessions for every stage.
%The stage is part of the state of the challenge and 1 by default.
%If notions allow for multiple stages,

%
%\begin{table} [h]
%\center
%\resizebox{0.45\textwidth}{!}{%
%  \begin{tabular}{ c c p{6cm}}
%
%Symbol & Name &Short description\\ \hline
%%$\mathsf{CR}_c$&limited number of challenge rows & $c$ communications in the two scenarios are allowed to differ.\\ \hline
%$R_{SR}$&Random Sender Receiver&One of the senders and one of the receivers of the challenge row are drawn randomly.
%For b=0 one of the adversary given sender-receiver pairs is drawn.
%For b=1 the sender is paired with the receiver of the other scenario.\\ %drawSenderReceiver
%$R_{XY}$&& analogous\\ \hline
%$T_S$&Twice Sender&The sender of the other scenario might be used when sending the second time (stage 2).
%For b=0 the same sender sends in both stages, for b=1 each sender sends in one of the stages.\\ 
%$T_R$&& analogous \\ \hline %switchSender
%$M_{SR}$&Mix Sender Receiver&Senders and receivers of the challenge row might be shuffled.
%For b=0 both communications of the first challenge row take place.
%For b=1 the communications take place with shuffled senders or receivers.\\ %addSenderReceiver
%$M_{XY}$&&analogous\\
%\end{tabular}}
% \caption{Complex Properties}
%  \label{tab:changes}
%\end{table}

%\paragraph{Defining those properties}

\begin{definition}[Property $T_S$]\label{def:complexProperties}
Let the given batches be $\underline{r}_b^a$ for instances $a \in \{0,1\}$ and scenarios $b \in \{0,1\}$,  $x$ the current stage, 
  $\mathsf{CR}$  the set of challenge row indexes, 
  $(u^a_0, {u'}^a_0)$ for both instances $a\in \{0,1\}$  be the sender-receiver-pairs of the first challenge row of the first scenario ($b=0$) \iflong in this challenge \fi in stage 1 and $(\tilde{u}^a_0,\tilde{u}'^a_0)$ the same pairs in stage 2.
Twice Sender $T_S$ is met, iff ($T_R$ analogous):
%\allowdisplaybreaks
\begin{align*}
  T_{S}:&\quad x=stage1~\land\\
   &\qquad{r_0^a}_{cr}=(\mathbf{u^a_0},  {u'}^{\:0}_0,m^1_{0_{cr}},aux^1_{0_{cr}})~\land \\
   &\qquad{r_1^a}_{cr}=(\mathbf{u^a_0},  {u'}^{\:0}_0,m^1_{0_{cr}},aux^1_{0_{cr}})\\[0.2em]
   \mathbf{\lor} &\quad x=stage2~\land\\
   &\qquad{r_0^a}_{cr}= (\mathbf{u^{a}_0}, \tilde{u}'^{\:0}_0, m^1_{0_{cr}},aux^1_{0_{cr}})~\land \\
   &\qquad{r_1^a}_{cr}= (\mathbf{u^{1-a}_0}, \tilde{u}'^{\:0}_0, m^1_{0_{cr}},aux^1_{0_{cr}})\\
     &\quad\forall cr \in \mathsf{CR} , a \in \{0,1\}&
\end{align*}
%\todo[inline]{The last cr has to skip every second cr.. How to write this?}

\end{definition}
%We do need message and aux fixed even if $a$ changes, otherwise adv could use this to figure out a and knowing a helps to distinguish the scenarios with less information here (e.g. which sender comes first, would then break M_{SR}
 Hence, we need to facilitate distinct stages for notions with the complex properties $T_S$ or $T_R$. Precisely, in step 2 of the game the adversary is additionally allowed to switch the stages.
 
 Note that the above definition can easily be extended to having more stages and hence, more than two messages for which the adversary needs to decide whether they have originated at the same sender.
 
This set of properties allows us to specify all privacy goals that have been suggested in literature as privacy notions and additionally all that we deem important. 
It is of course difficult to claim completeness, as future \acp{ACN} may define diverging privacy goals and novel observable properties (or: side-channels) may be discovered.

\iflong %ends before Notions begin
\vspace{-0.3cm}
\subsubsection{Sessions}\label{sec:sessions}
 \vspace{-0.3cm}
Some \ac{ACN} protocols, like e.g. Tor, use sessions. Sessions encapsulate sequences of communications from the same sender to the same receiver by using the same session identifier for them.  In our formalization, the adversary can pick this identifier as part of the auxiliary information.
However, in reality the adversary often does not have this capacity. Hence,  also in the formalization she should not be able to distinguish the scenarios just because she can identify that two messages are part of the same session or because the session identifier is leaked.

So, to model sessions, the auxiliary information of a communication is set to be the session ID ($sess$): $aux=sess$. 
In most communications, $sess$ is a number. Only for the session notions, we require special session IDs that correspond to the current challenge $\Psi$ in all challenge rows: $Ch\Psi$. In this way, they have to be the same in both scenarios and a concrete $sess$ is only used in one stage of one challenge.
 %
%  So, to model sessions, the auxiliary information of a communication is set to be the session ID ($sess$) and an extension to the session ID ($ID$): $aux=(sess, ID)$. Usually those IDs and extensions are numbers, only for the session notions, we require special session IDs and extensions. In this way, they have to be the same in both scenarios and one $sess$ and $ID$ combination is only used in one stage of one challenge.
% 
 The session identifier that is handed to the \ac{ACN} protocol model is a random number that is generated  by the challenger when a new $sess$ is seen. Hence, neither leaking (it is a random number) nor linking session identifiers (it will be picked new for every challenge and stage) will give the attacker an advantage.

  We formalize this in the following definition, where we also use `$\_$’ to declare that this part of a tuple can be any value.\footnote{E.g.
$\exists(u,m,\_) \in r$ will be true iff $\exists u': \exists(u,m,u') \in r$.}


%  \begin{table} [tbh]
%\center
%\resizebox{0.45\textwidth}{!}{%
%  \begin{tabular}{ l p{7cm}}
%
%Symbol &Description\\ \hline
%
%$\manySess{X}$ &  For every challenge and stage a new session is created.\\ %why not for every stage?
%$X$&Sessions are not restricted.\\ 
%\end{tabular}}
% \caption{Restriction options for sessions}
%  \label{tab:session}
%\end{table}

\begin{definition}[Sessions]\label{def:sessions}
Let $x$ be the stage and $u^a_0,u^a_1,u'^a_0,u'^a_1$ be the senders and receivers of the first challenge row of this challenge $\Psi$ and stage in instance $a \in \{0,1\}$.
Property $sess$ is met, iff for all $a\in \{0,1\}$:
{\footnotesize
\begin{align*}
  sess&: \forall (r^a_0,r^a_1)\in \mathsf{CR}(\underline{r}^a_0,\underline{r}^a_1):(r^a_0,r^a_1)=\\
  &\quad (u^a_0,u'^a_0,\_,(x, Ch\Psi) ),(u^a_1,u'^a_1,\_,(x,Ch\Psi)) 
\end{align*}
}
\end{definition}
\vspace{-0.3cm}
 As not all protocols use sessions, we allow to add sessions as an option to the notion $X$ abbreviated by $\manySess{X}$.% shown in Table \ref{tab:session}.

\iflong
\subsection{Corruption} \label{sec:advCap}
Some adversary capabilities like user corruption imply additional checks our challenger has to do. In reality for most ACNs the privacy goal can be broken for corrupted users, e.g. a corrupted sender has no unobservability. Hence, we include this adversary capability into our definition for the notion. As all properties are independent from the adversary capability, we add adversary capabilities as an option, that can be more or less restricted as shown in Table \ref{tab:corruption options}.

 \paragraph{Corruption} 
 We allow the adversary to corrupt users in some notions.  
 This has implications on the challenger, when a corrupt query or a batch query arrives.
 
   \begin{table} [t]
\center
\resizebox{0.35\textwidth}{!}{%
  \begin{tabular}{ l p{7cm}}

Symbol &Description\\ \hline

$X$&Adaptive corruption is allowed.\\%&Bohli\\
$\static{X}$ & Only static corruption of users is allowed.\\%& AnoA, Gelernter
$\noCorr{X}$ & No corruption of users is allowed.\\ \hline%& Hevia 
$X$&Corrupted users not restricted.\\
$\corrNoComm{X}$&Corrupted users are not allowed to be chosen as senders or receivers.\\
$\corrOnlyPartnerSender{X}$&Corrupted users are not  allowed to be senders.\\ 
$\corrOnlyPartnerReceiver{X}$&Corrupted users are not  allowed to be receivers.\\
$\corrStandard{X}$&Corrupted users send/receive identical messages in both scenarios.\\ 
\end{tabular}}
 \caption{Options for corruption and for corrupted communication}
  \label{tab:corruption options}
\end{table}

 
 \inlineheadingTwo{Check on corrupt queries}
 This check depends on whether the user corruption is adaptive, static, or not allowed at all.
  The default case for notion $X$ is adaptive corruption, i.e.
the adversary can corrupt honest users at any time. 
With static corruption $\static{X}$, the adversary has to corrupt a set of users before she sends her first batch. 
The third option, $\noCorr{X}$, is that no user corruption is allowed.
We denote the set of corrupted users as $\hat{U}$.
 

\begin{definition}[Corruption: Check on Corrupt Query]\label{def:corruptionCorrupt}
Let $\hat{U}$ be the set of already corrupted users, $u$  the user in the corrupt query and $subsequent$ be true iff at least one batch query happened. 
The following properties are met, iff:
{\footnotesize
\begin{align*}
  {corr}_{static}&: subsequent \implies u \in \hat{U} \\
  {corr}_{no}&: \perp  \quad \quad {corr}_{adaptive}: \top\\
\end{align*}
}
\end{definition}
\vspace{-2em}
\inlineheadingTwo{Check on batch queries}
As it would not make sense to protect the privacy of corrupted users, we need to assure that the adversary cannot distinguish the scenario because the behavior of corrupted users differs.  This is done by assuring equal behavior $corr$ or banning such users from communicating $\corrNoComm{corr},\corrOnlyPartnerSender{corr},\corrOnlyPartnerReceiver{corr}$.


\begin{definition}[Corruption: Check on Batch Query]\label{def:corruption}
The following properties are met, iff for all $a \in \{0,1\}$:
{\footnotesize
\begin{align*}
  \corrNoComm{corr}&: \forall (u,u',m,aux) \in \underline{r}^a_0\cup \underline{r}^a_1: S \not \in \hat{U} \land R \not \in \hat{U} \\
  \corrOnlyPartnerSender{corr}&: \forall (u,u',m,aux) \in \underline{r}^a_0\cup \underline{r}^a_1: u \not \in \hat{U} \\
  \corrOnlyPartnerReceiver{corr}&: \forall (u,u',m,aux) \in \underline{r}^a_0\cup \underline{r}^a_1: u' \not \in \hat{U}\\
  corr&: \forall \hat{u} \in \hat{U}:r^a_{0_i}=(\hat{u},\_,m,\_) \implies r^a_{1_i}=(\hat{u},\_,m,\_)\\
   &\quad \quad \quad \quad \land r^a_{0_i}=(\_,\hat{u},m,\_) \implies r^a_{1_i}=(\_,\hat{u},m,\_) \\
\end{align*}
}
\end{definition}
\vspace{-0.5cm}

Of course, other adversarial capabilities can be adjusted with other parts of the model (like the corruption of other parts of the \ac{ACN} with protocol queries).

\subsection{Quantification}\label{sec:challenges}
The aspects introduced in this section are based on the game and do not translate into the real world easily. However, they are useful for the analysis, since they quantify privacy.

\inlineheading{Challenge Complexity}
\todo[inline]{Why do we really want to do this?}
To quantify how different the scenarios are allowed to be, we add the concept of \emph{challenge complexity}. Challenge complexity is measured in
\textit{Challenge rows}, the pairs of communications that differ in the two scenarios as defined earlier. $c$ is the maximal allowed number of challenge rows  in the game. Additionally, we abbreviate the maximal allowed numbers of  challenge rows  per challenge to at most $\#cr$  as option to a notion $X$ with $X_{\mathsf{CR}_{\#cr}}$.

\example{Consider Alice using a protocol, that achieves $\bohliSSAc$ for one challenge row ($\bohliSSAc_{\mathsf{CR}_{1}}$), but not for two($\bohliSSAc_{\mathsf{CR}_{2}}$). This means in the case that Alice only communicates once, the adversary is not able to distinguish Alice from any other potential sender Charlie. However, if Alice communicates twice the regime might distinguish her existence from the existence of some other user.\todo{intersection attacks?}}

\begin{definition}[Challenge Complexity]\label{def:challengeComplexity}
Let $\#\mathsf{CR}$ be the number of challenge rows in this challenge so far, 
We say that the following property is met, iff:
 \allowdisplaybreaks
\begin{align*}
\mathsf{CR}_{\#cr}:& \#\mathsf{CR} \leq \#cr
\end{align*}
\end{definition}
 
 \inlineheading{Challenges Cardinality}
So far, we defined all aspects for one challenge.  We now bound the number of challenges to $n$, as the adversary potentially gains more information the more challenges are played. While challenge complexity defines a bound on the total number of differing rows within a single challenge, cardinality bounds the total number of challenges.
Communications belonging to a challenge are identified by the challenge number $\Psi$, which has to be between 1 and $n$ to be valid. The challenge number is a part of the auxiliary information of the communication  and is only used by the challenger, not by the protocol model.

This dimension of quantification can be useful for analysis, since for certain assumptions it is known, how the privacy of the $n$-challenge-case can be bounded in the privacy of the single-challenge-case (see Section \ref{advClass} for more information). 
 

\fi
\fi

\section{Privacy Notions}
\label{notions}

Given the properties above, we can now set out to actually express intuitive privacy goals as formal privacy notions.
We start by specifying sender unobservability as an example first, to give a general definition of our privacy notions after.
%With all fundamental principles defined, we can start building privacy notions from properties. We will give one formalization step by step. Since the other definitions work analogously, we define them all together. The informal understanding belonging to the notions is given in the next section together with an exemplary use case.
%This is done by defining which aspects valid adversarial queries have to satisfy, i.e. which information can leak. 
%Additionally, we give options for the assumed sessions, adversarial capability and quantification aspects. 

Recall the first game we defined in Section \ref{background}, which corresponds to sender unobservability ($\bohliSSAc$ = S(ender) $\lnot$ O(bservability)). There, in both scenarios something has to be sent, i.e. we need to specify that sending nothing is not allowed: \something. Further, both scenarios can only differ in the senders, i.e.  we also need the property that everything but the senders is equal: $\EveryButSender$. Hence, we define sender unobservability as $\bohliSSAc :=$\something$ \land \EveryButSender$.
\footnote{Technically $\EveryButSender$ already includes \something. However, to make the differences to other notions more clear, we decide to mention both in the definition.}

We define all other notions in the same way:

\begin{definition}[Notions]
Privacy notions are defined as boolean expression of the properties %and preprocessing methods into Algorithm \ref{TemplateAlpha}
 according to Table~\ref{NotionsDefinition}.
\end{definition}

 \begin{table}[htb]
\center
\resizebox{0.4\textwidth}{!}{%
  \begin{tabular}{ l l }

Notion&\iflong Aspects\else Properties \fi \\ \hline
$\loopixSRTPU$ &\something $ \land \EveryButSenderRec \land M_{SR}$  \\
$\anoaREL$ &\something$\land \EveryButSenderRec \land R_{SR}$ \\
$\newCONFWOL$ &\something $ \land \EveryButMsg$ \\
$\newCONF$ &\something $ \land \EveryButMsg \land |M| $ \\
$\heviaUL$&  \something$\land Q \land Q'$\\
$\bohliSA$& \something \\
$\heviaUO$& \nothing\\ \hline
$\bohliSSAc$& \something $\land \EveryButSender$\\
$\bohliSSUPc $& \something$\land \EveryButSender \land |U|$\\
$\bohliSWUPc$ &\something$\land \EveryButSender \land H$\\
$\bohliSPSc $&\something $\land \EveryButSender \land P$\\
$\bohliSSUUc$ &\something$\land \EveryButSender \land U$ \\
$\bohliSWUUc$ &\something $\land \EveryButSender \land U \land H$\\
$\bohliSANc $&\something $\land \EveryButSender \land U \land P$\\
$\bohliSWUc$ &\something $\land \EveryButSender \land Q$\\
$\bohliSWAc$ &\something $\land \EveryButSender \land Q \land P$\\
$\anoaUL$ &\something$\land \EveryButSender \land T_S $ \\
$\bohliRSAc$ \ etc.&analogous\\ \hline
\mbox{$\newAnoaSAWOL$}&\something $ \land \EveryButSenderMsg $ \\
\mbox{$\newAnoaSA$}&\something $ \land \EveryButSenderMsg \land |M| $ \\
$\newSAUO$ &\something $  \land \EveryButSenderMsg \land R_{SM}$ \\
$\newSA$&\something $  \land \EveryButSenderMsg \land M_{SM} $ \\
\mbox{$\anoaRA$} \ etc.&analogous \\ \hline
$\sgame{X'}$& Properties of $X'$, remove $\EveryButRec$ \\
\multicolumn{2}{c}{for $X' \in \{\bohliRSAc,$ $ \bohliRSUPc,$ $\bohliRWUPc,$ $\bohliRPSc,$ $\bohliRSUUc,$} \\
\multicolumn{2}{c}{$\bohliRWUUc,$ $\bohliRANc,$ $\bohliRWUc,$ $\bohliRWAc\}$}\\
$\rgame{X}$ &analogous \\ 
\iflong
 \hline
$\challengeRows{X}$& Properties of  $ X \land \mathsf{CR}_c$\\%) $\lor E$ \\
%$\oneSess{X}$& Properties of  $ X \land sess \land \mathsf{CR}_c$ \\
$\manySess{X}$&Properties of $X \land sess$\\

$\corrStandard{X}$, $\corrNoComm{X}$ \ etc.& $\land corr$, $\land  \corrNoComm{corr}$ \ etc.\\%\footnote{for all corruption options as defined in Table~\ref{tab:corruption options}}  \\
\fi
\end{tabular}}
 \caption{Definition of the notions\iflong for all corruption options as defined in Table~\ref{tab:corruption options}\fi. A description of simple properties was given in Table~\ref{tab:information}. }
  \label{NotionsDefinition}
\end{table} 

\iflong
Modeling the notions as a game, the respective challenger will check all aspects of the adversary's queries.
%The challenger will check for the aspects once receiving the relevant query. 
A complete description of the challenger can be found in Appendix \ref{sec:challenger}. 

Further, an example of how the definitions of aspects can be represented by using a challenge specific state, which the challenger maintains, is shown in Algorithm \ref{Challenger} and \ref{calcNewState}  in Appendix \ref{pseudocode}.
\else
Modeling the notions as a game, the respective challenger will check all aspects of the adversary's queries.
%The challenger will check for the aspects once receiving the relevant query. 
A complete description of the challenger can be found in Appendix \ref{sec:challenger}. 
\fi


%\todo[inline]{Thorsten to 5.1: ``a bit out of blue, break of story, rephrase to make easier to digest''}
\section{On the Choice of Notions}
\label{sec:choiceNotions}


The space of possible combinations of properties, and hence of conceivable privacy notions, naturally is large.
Due to that, we verified our selection of privacy goals by finding exemplary use cases.
Additionally, we approve the choice and the applicability of our definition  by analyzing the privacy goals of Loopix, an \ac{ACN} that was recently published.
We additionally verify that our privacy notions include those of previous publications that suggest frameworks based on indistinguishability games, and we provide a complete mapping in Section \ref{sec:ComparingFrameworks}.

%We verified the importance of the notions we formalized above by finding an exemplary use case for each of them (see Section \ref{sec:notionExamples}).
%Further, by analyzing the goals of a current \ac{ACN} we checked that current, practical proposals use similar goals (see Section \ref{sec:loopix}). %\todo[inline]{Loopix here or after other Frameworks? Can we sell Loopix like this?}
\iflong
\else
%  To assure that we cover most important notions, we checked that we include the notions of other frameworks\footnote{Notions of related frameworks are broken down to the observable information, excluding any inherent adversary model.} based on indistinguishability games. More details on how our notions map to other frameworks are depicted in Section \ref{sec:ComparingFrameworks}.
\fi

\subsection{Exemplary Use Cases for the Notions}
\label{sec:notionExamples}
We illustrate  our notions by continuing the example of an activist group trying to communicate in a repressive regime, although our notions are applicable in general. %can be applied in multiple contexts.% and publish date and time for their next demonstration in a repressive regime.

Recall the  general idea of an indistinguishability game from the examples in Section \ref{background}:
To prove that an \ac{ACN} hides certain properties, whatever is allowed to be learned in the actual \ac{ACN} must not help a game adversary to win, such that she is forced to win the game solely based on properties that are required to remain hidden.
Therefore, the information allowed to be disclosed cannot be used in the game and hence has to be kept identical in both scenarios.

Before giving examples, we want to order the notions. Hence, we group them semantically.
Our resulting clusters are shown as gray boxes in Figure \ref{fig:hierarchyColored}. %\ref{fig:clusterHierarchy} to group the notions. 
Horizontally, we categorize notions that focus on receiver or sender protection (Receiver Privacy Notions or Sender Privacy Notions, respectively) or treat both with the same level of importance (Impartial Notions).
Inside those categories we use clusters concerning the general leakage type: Both-side Unobservability means that neither senders, nor receivers or messages should be leaked.
Both-side Message Unlinkability means that it should neither be possible to link senders nor receivers to messages. In Sender Observability, the sender of every communication can be known, but not the message she sends or to whom she sends (Receiver and Message Observability analogous). In Sender-Message Linkability, who sends which message can be known to the adversary (Receiver-Message and Sender-Receiver Linkability analogous).
%We show the notions sorted in the clusters in Figure \ref{fig:hierarchyColored}.
\iflong
 \begin{table} [thb]
\center
\resizebox{0.4\textwidth}{!}{%
  \begin{tabular}{ c p{6cm}  }

Usage&Explanation\\ \hline
$D \in \{S,R,M\}$& Dimension $\in \{$Sender, Receiver, Message$\}$\\
Dimension $D$ not mentioned& Dimension can leak \\ 
Dimension $D$ mentioned &Protection focused on this dimension exists\\ \hline
$D \overline{O}$& not even the participating items regarding D leak,(e.g. $S\overline{O}$: not even $U$ leaks)\\
$DF \overline{L}$& participating items regarding D can leak, but not which exists how often (e.g. $SF\overline{L}$: $U$leaks, but not $Q$)\\
$DM \overline{L}$& participating items regarding D and how often they exist can leak ( e.g. $SM\overline{L}$: $U,Q$ leaks)\\ \hline
$X -Prop, $& like X but additionally Prop can leak\\
$Prop \in \{|U|,H,P,|U'|, H',P', |M| \}$&\\  \hline
$(D_1 D_2)\overline{O}$& uses $R_{D_1 D_2}$; participating items regarding $D_1,D_2$ do not leak, (e.g. $(SR)\overline{O}$: $R_{SR}$)\\ 
$(D_1 D_2)\overline{L}$& uses $M_{D_1 D_2}$; participating items regarding $D_1,D_2$ can leak, (e.g. $(SR)\overline{L}$: $M_{SR}$)\\ 
$(2D)\overline{L}$& uses $T_{D}$; it can leak whether two participating item regarding $D$ are the same,  (e.g. $\anoaUL$: $T_{S}$)\\ \hline
$\overline{O}$&short for $S \overline{O} R\overline{O} M\overline{O} $\\
$\heviaUL$& short for $ M\overline{O}(SM\overline{L}, RM\overline{L})$\\
$S\overline{O}\{X\}$& short for $S\overline{O} M\overline{O} X$\\
$D_1 X_1[ D_2 X_2]$& $D_1$ is dominating dimension, usually $D_1$ has more freedom, i.e. $X_2$ is a weaker restriction than $X_1$ \\ \hline
$C\overline{O}$& nothing can leak (not even the existence of any communication)\\
\end{tabular}}
 \caption{Naming Scheme}
  \label{Tab:NamingScheme}
\end{table}

We first want to explain our naming scheme, which we also summarize in Table \ref{Tab:NamingScheme}. Our notions consider three dimensions:  senders, messages and receivers.
 Each notion restricts amount of leakage on each of those dimensions. However, if one dimension can be leaked to the adversary, we do not mention this type. 
We use $\overline{O}$, short for unobservability, whenever the set of such existing items of this dimension cannot be leaked to the adversary.
 E.g. $S\overline{O}$ cannot be achieved if the set of senders $U$ is leaked. 
 We use some form of $\overline{L}$, short for unlinkability, if $U$ can be leaked, but some other property related to the item cannot. 
 E.g. we use $SF\overline{L}$ if the frequency $Q$ cannot be leaked and $SM\overline{L}$, if $Q$ can be leaked, but not the sender-message relation. 
  With a ``$- Prop$'' we signal that the property $Prop$ can additionally leak to the adversary. We distinguish those properties from $U$ and $Q$ used before as they give another leakage dimension (as illustrated later in the hierarchy).
 Further, we use $(SR)\overline{O}$ to symbolize that if not only one set, but both sets of senders and receivers ($U$ and $U'$) are learned the notion is broken. Analogously, in $(SR)\overline{L}$ both sets can be learned but the linking between sender and receiver cannot.
For the last missing complex property, we use $(2S)\overline{L}$ to symbolize that two senders have to be linked to be the same identity to break this notion.

For readability we also add some abbreviations: 
We use  $\overline{O}= S \overline{O} R\overline{O} M\overline{O} $ to symbolize unobservability on all three types and  we summarize the remaining types in $ M\overline{O}(SM\overline{L}, RM\overline{L})$ to $\heviaUL$. $C\overline{O}$ symbolizes the notion in which nothing is allowed to leak.
Further, we use curly brackets to symbolize that the message cannot be leaked $ S\overline{O}\{X\}= S\overline{O} M\overline{O} X$ and we also try to put the in our understanding non dominating part of the notion in brackets $S\overline{O} M\overline{O}= S\overline{O}[M\overline{O}]$.

\else
Table \ref{Tab:NamingScheme} of Appendix \ref{app:summaryNamingScheme} summarizes our naming scheme.
\fi
%\begin{figure}[htbp]
%  \centering
%  \includegraphics[width=0.45\textwidth]{images/clusterHierarchy.pdf}
%  \caption{Illustration of the used clusters}
%  \label{fig:clusterHierarchy}
%\end{figure}


%The adversary shall only win, if she learns something that is supposed to be private/protected.

%\todo[inline]{TODO: use words/descriptions in text, not symbols -> reduce cognitive load on reader}
\vspace{-0.3cm}
\subsubsection{Impartial Privacy Notions}
\vspace{-0.2cm}
These notions treat senders and receivers equally.

\inlineheading{Message Observability}
Messages' content can be learned in notions of this group, because messages are not considered confidential. Because the adversary in reality can learn the content, we have to avoid that she trivially wins the game by choosing different content. 
Hence, such notions use the property that the scenarios are identical except for the senders and receivers ($\EveryButSenderRec$) to ensure that the messages are equal in both scenarios. 

\example{One person of the activist group is already well known and communication with that person leads to persecution of Alice.}

Alice needs a protocol that hides whether a certain sender and receiver  communicate with each other; cf. Section \ref{sec:ComplexProperties} motivation of the complex property $M_{SR}$.
The resulting notion is \emph{\loopixSRTPULong \ ($\loopixSRTPU$)}.

\exampleCont{Only few people participate in the protocol. Then, already using the protocol  to receive (send) something, when the well known activist is acting as sender (receiver) threatens persecution. }

Alice needs a protocol that hides whether a certain sender and receiver actively participate at the same time or not; cf. Section \ref{sec:ComplexProperties} motivation of the complex property $R_{SR}$.
The resulting notion is \emph{\anoaRELLong\  ($\anoaREL$)}.


\inlineheading{Sender-Receiver Linkability (Message Confidentiality)}
Senders and receivers can be learned  in notions of this group, because they are not considered private.
Hence, such notions include the property that the scenarios are identical, except for the messages ($\EveryButMsg$) to ensure that the sender-receiver pairs are equal in both scenarios.

\example{Alice wants to announce her next demonstration. (1) Alice does not want the regime to learn the content of her message and block this event. (2) Further,  she is afraid that the length of her messages could make her suspicious, e.g. because activists tend to send messages of characteristic length.}


In (1) Alice needs a protocol that  hides the content of the messages. However, the adversary is allowed to learn all other attributes,
especially also the length of the message.
Modeling this situation, the scenarios may differ solely in the message
content, all other attributes have to be identical in both scenarios, as
they may not help the adversary distinguish between them.
Beyond the above described $\EveryButMsg$, we thus also have to request that the
length of the messages $|M|$ is identical in both scenarios.
The resulting notion is  \emph{\newCONFLong\ ($\newCONF$)}\footnote{We stick to our naming scheme here, although we would commonly call this confidentiality.}.

In the second case (2), the protocol is required to hide the length of the message.
The length of the messages thus may differ in the two scenarios, as the
protocol will need to hide this attribute. Hence, we remove the restriction that the message length has to be equal in both scenarios $|M|$ from the above notion and end up with \emph{\newCONFWOLLong\ $\newCONFWOL$}.

\iflong
\inlineheading{Both-Side Message Unlinkability}
Notions of this group are broken if the sender-message or receiver-message relation leaks.

\example{The activists know  that their sending and receiving frequencies are similar to regime supporters and that using an \ac{ACN} is in general not forbidden, but nothing else. Even if the message's content and length ($\newCONFWOL$) and the sender-receiver relationship ($\loopixSRTPU$)  is hidden, the regime might be able to distinguish uncritical from critical communications, e.g. whether two activists communicate  ``Today'' or  innocent users an innocent message.  In this case, the regime might learn that currently many critical communications take place and improves its measures against the activists.}

In this case, the activists want a protocol that hides the communications, i.e. relations of sender, message and receiver. However, as using the protocol is not forbidden and their sending frequencies are ordinary, the adversary can learn which users are active sender or receiver and how often they sent and receive. Modeling this, the users need to have the same sending and receiving frequencies in both scenarios $Q,Q'$, since it can be learned. However, everything else needs to be protected and hence, can be chosen by the adversary. This corresponds to the notion  \emph{\heviaULLong \ ($\heviaUL$)}.
\fi


\inlineheading{Both-Side Unobservability}
Even the activity of a certain sender or receiver is hidden in notions of this group.

\exampleCont{It is a risk for the activists, if the regime can distinguish between two leading activists exchanging the message ``today'' and two loyal regime supporters exchanging the message ``tomorrow''.}

 In this case, Alice wants to disclose nothing about senders, receivers, messages or their combination . However, the adversary can learn the total number of communications happening in the \ac{ACN}. Modeling this, we need to assure that for every communication in the first scenario exists one in the second. We do this prohibiting the use of the empty communication with property \something. This results in the notion \emph{\bohliSALong \ ($\bohliSA$)}.

\example{The regime knows that a demonstration is close, if the total number of communications transmitted over this protocol increases. Then it prepares to block the upcoming event.}

To circumvent this, Alice needs a protocol  that additionally hides the total number of communications. Modeling this, we need to allow the adversary to pick any two scenarios. Especially, also using the empty communication  $\Diamond$ is allowed. This is represented in the property that nothing has to be equal in the two scenarios: \nothing\  and results in the notion \emph{\heviaUOLong \ ($\heviaUO$)}.
Note, that this is the only notion, where the existence of a communication is hidden. All other notions include \something\ and hence do not allow for the use of the empty communication.


%\todo[inline]{For all following notions, the mere existence of a communication is allowed to leak.
%Hence for all further notions in both scenarios the number of communications (sent messages) needs to be equal,  $\Diamond$ is nor allowed in these scenarios.}

\subsubsection{Sender (and Receiver) Privacy Notions}
\vspace{-0.2cm}
These notions allow a greater freedom in picking the senders (resp.
receivers: analogous notions are defined for receivers.).

\inlineheading{Receiver-Message Linkability}
The receiver-message relation can be disclosed in notions of this group.
Hence, such notions include the property that the scenarios are identical except for the senders ($\EveryButSender$) to ensure the receiver-message relations are equal in both scenarios.

In \emph{\bohliSWUcLong \ ($\bohliSWUc$)} additionally the total number of communications and how often each user sends can be learned.
However, especially who sends which message is hidden.
In \emph{\bohliSSUUcLong } \emph{($\bohliSSUUc$)} additionally the set of users and the total number of communications can be disclosed.
However, especially how often a certain user sends is hidden, since it can vary between the two scenarios.
In \emph{\bohliSSAcLong \ ($\bohliSSAc$)}, the total number of communications can additionally be disclosed.
 However, especially the set of active senders $U_b$ is hidden.


If a notion further includes the following abbreviations, the following information can  be disclosed as well:
\begin{itemize}
 \item \emph{with User Number Leak}  ($-|U|$): the number of senders that send something in the scenario
\item \emph{with Histogram Leak}  ($-H$):  the histogram of how many senders send how often 
\item \emph{with Pseudonym Leak}  ($-P$): which messages are sent from the same user 
\end{itemize} \vspace*{-\baselineskip}
%In all those notions everything that is allowed to leak will be checked to be equal in both scenarios.

\exampleSpec{Alice is only persecuted when the regime can link a message with compromising content to her {\normalfont -- she needs a protocol that at least provides $\bohliSWAc$.} 
However, since such a protocol does not hide the message content, the combination of all the messages she sent, might lead to her identification. {\normalfont Opting for a protocol that additionally hides the message combination ($P$), i.e. provides $\bohliSWUc$,  can protect her from this thread.} \\
Further, assuming most users sent compromising content, and Alice's message volume is high, the regime might easily suspect her to be the origin of some compromising messages even if she is careful that the combination of her messages is not reidentifying her {\normalfont - she  needs a protocol that does not disclose her sending frequencies ($Q$) although the combination of her messages ($P$) might be learned, i.e. achieving $\bohliSANc$.}
However, Alice might fear disclosing the combination of her messages {\normalfont - then she needs a protocol achieving at least $\bohliSWUUc$, which hides the frequencies ($Q$) and the message combination ($P$), but discloses the sending histogram, i.e. how many people sent how many messages ($H$).}
However, if  multiple activist groups use the \ac{ACN} actively at different time periods, disclosing the sending histogram $H$ might identify how many activist groups exist and to which events they respond with a more active communication {\normalfont - to prevent this she needs a protocol that hides the frequencies $Q$ and the histogram $H$, i.e. provides $\bohliSSUUc$.} \\
 %only very few activists are very active, this information might lead the regime to the number of core activists and  this might with external knowledge lead to identifying those. }
Further, not only sending a certain content, but also being an active sender (i.e. being in $U$) is prosecuted {\normalfont she might want to pick a protocol with at least $\bohliSPSc$. 
Again if she is afraid that leaking $P$ or $H$ together with the expected external knowledge of the regime leads to identifying her, she picks the corresponding stronger notion.}
If the regime knows that mostly activists send in the \ac{ACN} and learns that the  number of active senders is high, it blocks the \ac{ACN}. 
{\normalfont In this case at least $\bohliSSAc$ should be picked to hide the number of senders ($|U|$).}}

\example{ For the next protest, Alice sends two messages: (1) a location, and (2) a time. If the regime learns that both messages are from the same sender, they will block the place at this time even if they do not know who sent the messages.} 
Alice then needs a protocol that hides whether two communications have the same sender or not. We already explained how to model this with complex property $T_{S}$ in  Section \ref{sec:ComplexProperties}.
The resulting notion is \anoaULLong ($\anoaUL$).


%In \emph{\loopixSUONeLong} ($\loopixSUONe$) the adversary is additionally to the restrictions of $\bohliSSAc$ restricted not to use the sender of the first scenario in the first challenge row as a sender in the second scenario.
%\todo[inline]{Why should we define this notion?}
%: \bohliRSAcLong \ ($\bohliRSAc$), \bohliRSUUcLong\  ($\bohliRSUUc$), \bohliRWUcLong \ ($\bohliRWUc$), etc.
\iflong

\inlineheading{Receiver Observability}
In notions of this group the receiver of each communication can be learned.
Hence, such notions include the property that the scenarios are equal except for the senders and messages ($\EveryButSenderMsg$) to ensure that they are equal in both scenarios.

\example{Consider not only sending real messages is persecuted, but also the message content or any combination of senders and message contents is exploited by the regime. If the regime e.g. can distinguish activist Alice sending ``today'' from regime supporter Charlie sending ``see u'', it might have learned an information the activists would rather keep from the regime.  Further, either (1) the activists know that many messages of a certain length are sent or (2) they are not sure that  many messages of a certain length are sent.}%\todo[inline]{is  ``valuable'' a strange expressions, there? Underlined by Thorsten...}

In case (1), Alice needs a \ac{ACN}, that hides the sender activity, the message content and their combination. However, the adversary can especially learn the message length. Modeling this, beyond the above described $\EveryButSenderMsg$, the message lengths have to be equal $|M|$. This results in the notion  \emph{\newAnoaSALong}  ($\newAnoaSA$).
Note that in $\newAnoaSA$ the properties of $\newCONF$ are included and further the senders are allowed to differ in the two scenarios.
The second case (2) requires a protocol that additionally hides the message length. Hence, in modeling it we remove the property that the message lengths are equal $|M|$ from the above notion. This results in \emph{\newAnoaSAWOLLong}  ($\newAnoaSAWOL$).


\example{ Alice's demonstration is only at risk if the regime can link a message with a certain content to her as a sender with a non negligible probability.} 
Then at least \emph{\newSALong\  ($\newSA$)}, which is defined analogous to $\loopixSRTPU$ is needed. 
\exampleCont{However, $\newSA$ only allows Alice to claim that not she, but Charlie sent a critical message $m_a$ and the regime cannot know or guess better. Now assume that Dave is also communicating, then the regime might be able to distinguish Alice sending $m_a$, Charlie $m_c$ and Dave $m_d$ from Alice sending $m_d$, Charlie $m_a$ and Dave $m_c$. In this case, it might not even matter that Alice can claim that Charlie possibly sent her message. The fact that when comparing all three communications that possibly happened, Alice is more likely to have sent the critical message $m_a$ means a risk for her.}

 To circumvent this problem Alice needs a protocol that not only hides the difference between single pairs of users, but any number of users. Modeling this, instead of the complex property $M_{SM}$, we need to restrict that the active senders' sending frequencies are equal.
 %Analogous to $\loopixSRTPU$, in $\newSA$ the sender-message pairs have to be guessed.
%and in \emph{\newRALong\  ($\newRA$)} the receiver-message .

\example{In another situation our activists already are prosecuted for being a sender while a message with critical content is sent. }

In this case at least  \emph{\newSAUOLong\  ($\newSAUO$)}, which is defined analogous to $\anoaREL$ is needed.
 %Analogous to $\anoaREL$, in $\newSAUO$ the sender-message existence has to be guessed.
% and in \emph{\newRAUOLong\  ($\newRAUO$)} the receiver-message existence .

Analogous notions are defined for receivers.

\inlineheading{Both-Side Unlinkability}
As explained with the example before in the case that Alice does not want any information about senders, receivers and messages or their combination to leak, she would use $\bohliSA$. However, the privacy in this scenario can be tuned down, if she assumes that the regime does not have certain external knowledge or that the users are accordingly careful. As explained for the Sender Notions with Receiver-Message Linkability before, in this case we might decide to allow $U', |U'|,Q',H',P'$ to leak.

If a notion $X \in \{\bohliRSAc, \bohliRSUPc, \bohliRWUPc, \bohliRPSc,\bohliRSUUc,\bohliRWUUc,\bohliRANc,\bohliRWUc,\bohliRWAc\}$ is extended to \emph{Sender Unobservability by X} \emph{($ \sgame{X}$)}, the leaking of the sender-message relation is removed.
This is done by removing $\EveryButRec$.
 Since the attacker now has a greater degree of freedom in choosing the senders and is (if at all) only restricted in how she chooses the receivers and messages, this is a special strong kind of Sender Unobservability.
 Analogous notions are defined for receivers.\footnote{Note that $\sgame{\bohliRSAc}=\rgame{\bohliSSAc}=\bohliSA$.}


\subsubsection{Options}
Options, which can be combined arbitrarily to all so far explained notions, are sessions, corruption and challenge complexity. Their relation to the real world resp. to easier analysis can be found in Sections \ref{sec:sessions}, \ref{sec:advCap} and \ref{sec:challenges}.

\else
Due to the page limits the examples for the remaining notions can be found in Appendix \ref{app:examples}.
\fi

%\subsection{Remark}
%Most of the defined notions are adapted versions of notions from other frameworks.
%\todo[inline]{Stress that this task to make the notions of other frameworks compatible is not trivial?}Section \ref{sec:mappingpapers} explains how the notions of the other papers can be translated to our notions (and with this shows which notions were adapted to get to our new notions).


==> sections/proofs/OthersToOur.tex <==

\inlineheading{Bohli}


\inlineheading{Hevia}


\inlineheading{Gelernter}
Most notions follow from the mapping of Hevia's to our notions. 

\inlineheading{AnoA}

